AC-DC: Adaptive Ensemble Classification for Network Traffic Identification

Accurate and efficient network traffic classification is important for many network management tasks, from traffic prioritization to anomaly detection. Although classifiers using pre-computed flow statistics (e.g., packet sizes, inter-arrival times) can be efficient, they may experience lower accuracy than techniques based on raw traffic, including packet captures. Past work on representation learning-based classifiers applied to network traffic captures has shown to be more accurate, but slower and requiring considerable additional memory resources, due to the substantial costs in feature preprocessing. In this paper, we explore this trade-off and develop the Adaptive Constraint-Driven Classification (AC-DC) framework to efficiently curate a pool of classifiers with different target requirements, aiming to provide comparable classification performance to complex packet-capture classifiers while adapting to varying network traffic load. AC-DC uses an adaptive scheduler that tracks current system memory availability and incoming traffic rates to determine the optimal classifier and batch size to maximize classification performance given memory and processing constraints. Our evaluation shows that AC-DC improves classification performance by more than 100% compared to classifiers that rely on flow statistics alone; compared to the state-of-the-art packet-capture classifiers, AC-DC achieves comparable performance (less than 12.3% lower in F1-Score), but processes traffic over 150x faster.

==> future.tex <==
\section{Future Work}\label{sec:future_work}
\paragraph{Expanding Evaluation Beyond Header Level Features.}
Our present evaluation solely employs packet header-level features
to execute classification tasks, serving as a preliminary introduction to
an alternative method of implementing adaptive ensemble classification
in network scenarios. However, we plan to expand our evaluation by
incorporating additional network features,
including finer-grained bit-level features, derived features, and cross layer features.
By increasing the feature space, we aim to achieve a finer-grained balance between
performance and efficiency. We will test the robustness of our framework
as we expand the feature space to verify its effectiveness.
 
\paragraph{Attaching {\sysname} to Ensemble-Structured Models.}
{\sysname} primarily addresses the bottleneck in preprocessing efficiency
in comparison to approaches that utilize ensemble methods to aggregate multiple
learning algorithms. However, it is possible to augment {\sysname} with traditional
ensemble techniques to create a classifier that is optimized for efficiency
at both stages of the classification pipeline. This is plausible because,
by varying the feature requirements, specific machine learning models may be
better suited to the selected features than others. A hybrid approach that
combines both methods may result in even better performance and efficiency.

\paragraph{Applying {\sysname} to Encrypted Network Traffic.}
Increasing levels of encryption presents a challenge for traditional machine learning classifiers, as they are typically unable to interpret the content of the traffic.
Thus applying {\sysname} to network traffic under different levels of encryption
is another potential area of exploration. The flexibility in {\sysname}'s feature requirements
can help to mitigate the risk of overfitting to a specific set of features,
which may be more likely to occur with encrypted traffic where the underlying
features may be less well understood.
